DAHash: Distribution Aware Tuning of Password Hashing Costs

An attacker who breaks into an authentication server and steals all of the cryptographic password hashes is able to mount an offline-brute force attack against each user's password. Offline brute-force attacks against passwords are increasingly commonplace and the danger is amplified by the well documented human tendency to select low-entropy password and/or reuse these passwords across multiple accounts. Moderately hard password hashing functions are often deployed to help protect passwords against offline attacks by increasing the attacker's guessing cost. However, there is a limit to how "hard" one can make the password hash function as authentication servers are resource constrained and must avoid introducing substantial authentication delay. Observing that there is a wide gap in the strength of passwords selected by different users we introduce DAHash (Distribution Aware Password Hashing) a novel mechanism which reduces the number of passwords that an attacker will crack. Our key insight ishat a resource-constrained authentication server can dynamically tune the hardness parameters of a password hash function based on the (estimated) strength of the user's password. We introduce a Stackelberg game to model the interaction between a defender (authentication server) and an offline attacker. Our model allows the defender to optimize the parameters of DAHash e.g., specify how much effort is spent to hash weak/moderate/high strength passwords. We use several large scale password frequency datasets to empirically evaluate the effectiveness of our differentiated cost password hashing mechanism. We find that the defender who uses our mechanism can reduce the fraction of passwords that would be cracked by a rational offline attacker by around 15%.

==> sections/background.tex <==
% !TEX root = main.tex

%\section{Password Distribution}
%\jenote{We want to start more basic then this. We assume that there is a distribution over user chosen passwords $\mathcal{P}$ and we use $p_i$ to denote the probability of $pwd_i$ --- the $i$'th most popular password. Thus, we have $p_1 \geq p_2 \geq \ldots $ and $\sum_i p_i = 1$. We assume that each user $u$ samples $pwd_u$ from this distribution. The attacker know the distribution over passwords, but not the specific password $pwd_u$. The distribution can approximated using empirical datasets. In particular, given a dataset of $N$ user passwords the corresponding password frequency list is simply a list of numbers $f_1 \geq f_2 \geq \ldots $ where $f_i$ is the number of users who selected the $i$th most popular password in the dataset --- note that $\sum_{i} f_i = N$. We can use the frequency list to empirically estimate $\tilde{p}_i \approx \frac{f_i}{N}$. \\
%A password frequency list can usually be more compactly represented as a sequence of tuple $(f_1,c_1),(f_2,c_2),\ldots$ with $f_i \geq f_{i+1}$. Here, the tuple $(f_i,c_i)$ indicates that there are $c_i$  distinct passwords each of which was observed exactly $f_i$ times --- note that $N= \sum_i f_i \times c_i$ when we use the compact representation. We will follow this view in the paper and assume that the distribution is specified as a list of $n'$ tuples $(p_i,c_i)$. In our experiments we use the empirical estimate
% $$p_i = \frac{f_i}{N}$$
%of $p_i$. We typically have $n' \ll N$ in empirical datasets e.g.,  for the LinkedIn dataset we have $N \geq 1.7 \times 10^8$ while $n' = 3639$. Thus, an algorithm whose running time scales with $n'$ is much faster than an algorithm whose running time scales with $N$. 
%  }


We let $\mathcal{P} = \{pw_1,pw_2,\ldots,\}$ be the set of all possible user-chosen passwords. We will assume that passwords are sorted so that $pw_i$ represents the $i$'th most popular password. Let $\Pr[pw_i]$ denote the probability that a random user selects password $pw_i$ we have a distribution over $\mathcal{P}$ with $\Pr[pw_1] \geq \Pr[pw_2] \geq \ldots $ and $\sum_i \Pr[pw_i] = 1$.  Given a user $u$ we will also use $pw_u$ to denote the password selected by this user. We assume that the attacker knows the distribution over $\mathcal{P}$ from which the password is selected, but does not know the particular password $pw_u$. In particular, we assume that the attacker knows $pw_i$ and $\Pr[pw_i]$ for each $i \geq 1$. We argue that it is a reasonable assumption because the attacker will have access to a massive amount of training data from prior password breaches and can also use sophisticated tools such as Probabilistic Context Free Grammars~\cite{SP:WAMG09,SP:KKMSVB12,NDSS:VerColTho14}, Markov Chain Models~\cite{NDSS:CasDurPer12,Castelluccia2013,SP:MYLL14,USENIX:USBCCKKMMS15}  and even neural networks~\cite{USENIX:MUSKBCC16} to generate likely password guesses (approximately accurate). Furthermore, an attacker who is trying to crack all passwords in the dataset $D$ can simply keep track of the passwords that s/he has already cracked along with their frequency. Any password that has already been observed in the dataset is likely to be repeated. For example, the breached LinkedIn dataset contained $170+$ million passwords, but only $12.29\%$ of those passwords were unique (chosen by only one user).
 %such that $N= \sum_i f_i \times c_i$. Here, the tuple $(f_i,c_i)$ 

 %(suppose $n’$ such tuples are listed in descending order of $f_i$), where $f_i$ is appearance frequency of certain passwords and $c_i$ is the corresponding observations. Thus $(f_i,c_i)$  can be interpreted as there are $c_i$ distinct passwords each of which appears $f_i$ times in the dataset of interest --- note that $N= \sum_i f_i \times c_i$ when we use the compact representation. We will follow this view in the paper and assume that the distribution is specified as a list of $n'$ tuples $(p_i,c_i)$. In our experiments we use the empirical estimate
 %$$p_i = \frac{f_i}{N}$$
% where $$p_1>p_2>\cdots p_{n’}.$$








%asume this is true, justify assumption
%\subsection{Empirical Passwords Data Representation}
%%\jenote{We want to start more basic then this. We assume that there is a distribution over user chosen passwords $\mathcal{P}$ and we use $p_i$ to denote the probability of $pwd_i$ --- the $i$'th most popular password. Thus, we have $p_1 \geq p_2 \geq \ldots $ and $\sum_i p_i = 1$. We assume that each user $u$ samples $pwd_u$ from this distribution. The attacker know the distribution over passwords, but not the specific password $pwd_u$. The distribution can approximated using empirical datasets. In particular, given a dataset of $N$ user passwords the corresponding password frequency list is simply a list of numbers $f_1 \geq f_2 \geq \ldots $ where $f_i$ is the number of users who selected the $i$th most popular password in the dataset --- note that $\sum_{i} f_i = N$. We can use the frequency list to empirically estimate $\tilde{p}_i \approx \frac{f_i}{N}$. \\
%%A password frequency list can usually be more compactly represented as a sequence of tuple $(f_1,c_1),(f_2,c_2),\ldots$ with $f_i \geq f_{i+1}$. Here, the tuple $(f_i,c_i)$ indicates that there are $c_i$  distinct passwords each of which was observed exactly $f_i$ times --- note that $N= \sum_i f_i \times c_i$ when we use the compact representation. We will follow this view in the paper and assume that the distribution is specified as a list of $n'$ tuples $(p_i,c_i)$. In our experiments we use the empirical estimate
%% $$p_i = \frac{f_i}{N}$$
%%of $p_i$. We typically have $n' \ll N$ in empirical datasets e.g.,  for the LinkedIn dataset we have $N \geq 1.7 \times 10^8$ while $n' = 3639$. Thus, an algorithm whose running time scales with $n'$ is much faster than an algorithm whose running time scales with $N$. 
%%  }
%  
%We assume that there is a distribution over user chosen passwords $\mathcal{P}$ and we use $p(pwd_i)$ to denote the probability of $pwd_i$ --- the $i$'th most popular password. Thus, we have $p(pwd_1) \geq p(pwd_2) \geq \ldots $ and $\sum_i p(pwd_i) = 1$. We assume that each user $u$ samples $pwd_u$ from this distribution. The attacker know the distribution over passwords, but not the specific password $pwd_u$. The distribution can be approximated using empirical datasets. In particular, given a dataset of $N$ user passwords the corresponding password frequency list is simply a list of numbers $f_1 \geq f_2 \geq \ldots $ where $f_i$ is the number of users who selected the $i$th most popular password in the dataset --- note that $\sum_{i} f_i = N$. We can use the frequency list to empirically estimate $\tilde{p}_i \approx \frac{f_i}{N}$.
%
%A password frequency list can usually be more compactly represented as a sequence of tuple $(f_i,c_i)$ (suppose $n’$ such tuples are listed in descending order of $f_i$), where $f_i$ is appearance frequency of certain passwords and $c_i$ is the corresponding observations. Thus $(f_i,c_i)$  can be interpreted as there are $c_i$ distinct passwords each of which appears $f_i$ times in the dataset of interest --- note that $N= \sum_i f_i \times c_i$ when we use the compact representation. We will follow this view in the paper and assume that the distribution is specified as a list of $n'$ tuples $(p_i,c_i)$. In our experiments we use the empirical estimate
% $$p_i = \frac{f_i}{N}$$
% where $$p_1>p_2>\cdots p_{n’}.$$
%
%We say passwords with the same probability belong to a \emph{equivalence class}. Then $c_i$ can be interpreted as the cardinality of equivalence class $i$ (the number of passwords in that equivalence class). Compact representation forms as $(f_i,c_i)$ and $(p_i,c_i)$ allow us to view passwords with the same probability as a whole instead of individually.  We typically have $n' \ll N$ in empirical datasets e.g.,  for the LinkedIn dataset we have $N \geq 1.7 \times 10^8$ while $n' = 3639$. Thus, an algorithm whose running time scales with $n'$ is much faster than an algorithm whose running time scales with $N$. 



==> sections/goodturing.tex <==
% !TEX root = ../main.tex


